MTS2Graph: Interpretable Multivariate Time Series Classification with Temporal Evolving Graphs

Conventional time series classification approaches based on bags of patterns or shapelets face significant challenges in dealing with a vast amount of feature candidates from high-dimensional multivariate data. In contrast, deep neural networks can learn low-dimensional features efficiently, and in particular, Convolutional Neural Networks (CNN) have shown promising results in classifying Multivariate Time Series (MTS) data. A key factor in the success of deep neural networks is this astonishing expressive power. However, this power comes at the cost of complex, black-boxed models, conflicting with the goals of building reliable and human-understandable models. An essential criterion in understanding such predictive deep models involves quantifying the contribution of time-varying input variables to the classification. Hence, in this work, we introduce a new framework for interpreting multivariate time series data by extracting and clustering the input representative patterns that highly activate CNN neurons. This way, we identify each signal's role and dependencies, considering all possible combinations of signals in the MTS input. Then, we construct a graph that captures the temporal relationship between the extracted patterns for each layer. An effective graph merging strategy finds the connection of each node to the previous layer's nodes. Finally, a graph embedding algorithm generates new representations of the created interpretable time-series features. To evaluate the performance of our proposed framework, we run extensive experiments on eight datasets of the UCR/UEA archive, along with HAR and PAM datasets. The experiments indicate the benefit of our time-aware graph-based representation in MTS classification while enriching them with more interpretability.

==> images/Algorithem1.tex <==
\begin{algorithm}[tb] 
\caption{Extraction of the MHAP}
\label{alg:MHAPsudocode}
\begin{algorithmic}[1]
\Require{$X_{train}$:= Multivariate time series data} 
\Ensure{MHAP representative patterns for each layer and layer's channel, MCMHAP}
\State Model $\longleftarrow$ {Training($X_{train}$)}
\For{$sample$ \texttt{in $X_{train}$}}  
    \State $signal_{train}$ = IS($sample$)

\For{$l$ \texttt{in Model\_layers}}
\For{$c$ \texttt{in $l$}}
    %\For{$s$ \texttt{in $signal_{train}$}}
    \State $HAN = [\forall n \in [1, N_{l,c}] \; where\; A(n) \geq T_{l,c}]$
    \State $MHAP = [SRF(signal_{train}) \;of \;HAN's]$
    \State $MHAP_{list}.add(MHAP)$ 
    \EndFor
\EndFor
\EndFor
\State CMHAP$\longleftarrow$$\{K_{shape}(MHAP_{list})\}$

%\State $GP_{list}.add(MCPHAP)$
%\State $x_{test} = X_{test}$ \Comment{Get an example from test data}
\State $MCMHAP_{list}.add(Median(CMHAP))$
\State \Return {$MHAP_{list}$, $MCMHAP_{list}$}
\end{algorithmic}
\end{algorithm}


==> images/Algorithem2.tex <==
\begin{algorithm}[tb] 
\caption{Time-aware MHAP Evolution Graph}
\label{alg:graphsudo}
\begin{algorithmic}[1]
\Require{$X_{train}$, $MCMHAP$} 
\Ensure{Time-aware Evolution Graph}
\For{l in \texttt{Model\_layers}}
    \State Initialize a graph $g$ with $n$ nodes \Comment{$n$ := size($MCMHAP_l$)} 
    \For{$s$ \texttt{in $X_{train}$}}  
        \State $signal_{train}$ = IS($sample$)
        
        \State $MHAP$ := GetHighActivePeriods($s$)
        \State Assign $MCMHAP(MHAP)$
        \For{all adjacent MHAP in $s$} \Comment{nodes $n_{i}$, $n_{i+1}$} %are $MCMHAP(MHAP)$}
             \State Add directed edge $e_{i,i+1}$
        \EndFor
    \EndFor
    \State $Graph_{list}.add(g)$
\EndFor
\State Initialize a graph $G$ with all graphs from $Graph_{list}$
\For{$g$ in $Graph_{list}$}
    \For{$n$ in $g$}
        \State Add directed edge to $n$ corresponding previous layer graph $MHAPs$ 
    \EndFor
\EndFor
\State \Return {$G$}
\end{algorithmic}
\end{algorithm}


==> images/table1.tex <==
\begin{table}[tb]
\caption{The statistics of the eight selected datasets from Baydogan’s multivariate time series archive, with HAR and PAM datasets.}
\centering
\begin{tabular}{lcccc}
 \toprule
 
 Dataset  & TS-length & Classes & Dimensions & \#samples  \\
\hline
 UWave &  $315$  & $8$& $3$  & $4478$ \\
ArabicDigits &  $93$  & $10$  & $13$  &$8800$  \\
AUSLAN & $136$ & $95$ & $22$& $2565$ \\
Libras  &$45$& $15$ & $2$ & $360$  \\
ECG & $152$ & $2$ & $2$  &$200$ \\
%KickVsPunch & 841 & 2 & 62 & 16 & 10\\
NetFlow & $997$& $2$ & $4$  & $1337$  \\
Wafer & $198$  & $2$ & $6$ & $1194$     \\
CharacterTrajectories & $205$ & $20$  & $3$ & $2858$ \\
HAR & $206$  & $6$ & $3$ & $10,299$ \\
PAM	 &  $600$  & $8$& $17$  & $5,333$\\

 \bottomrule
\end{tabular} \label{table0:archive}
\end{table}

==> images/table2.tex <==
\begin{table*}[tb]
\caption{Comparison of classification performance on the selected eight datasets. The best accuracy among all models are bold.}
\centering
\begin{tabular}{l|ccccr}
\hline
 Dataset  & FCN  &  ResNet   & MCDCNN & Encoder & MTS2Graph\\
\hline
UWave &  \textbf{0.93}  &0.92 &0.84&0.90&\textbf{0.93} \\
ArabicDigits &\textbf{0.99}&\textbf{0.99}&0.95&0.98&0.96 \\
AUSLAN &\textbf{0.97}&\textbf{0.97}&0.85&0.93&0.95\\
Libras  &\textbf{0.96}&0.95&0.65&0.78&0.93\\
ECG &0.87 &0.86&0.5&0.87&\textbf{0.90} \\
KickVsPunch &0.54&0.53&0.56&0.61&0.54 \\
NetFlow &\textbf{0.89}&0.62&0.77&0.63&0.87  \\
Wafer &\textbf{0.98}&\textbf{0.98}&0.65&\textbf{0.98}&\textbf{0.98}\\
\hline
\end{tabular} \label{table0:accuercy}
\end{table*}

==> images/table_term.tex <==
\begin{table}[tb]
\caption{Definitions of the frequent terminologies used in this paper.}
\centering
\begin{tabular}{llc}
\toprule
 
Termoenology  & Definition  \\
\hline
MTS& Multivariate Time Series \\
IS& Input Set \\
HAN&Highly Activated Neurons\\
MHAP& Multivariate highly activated period \\
SRF&Signal Receptive Field\\
CMHAP& Clustered Multivariate highly activated period \\
MCMHAP&Median Clustered Multivariate highly activated period\\


 \bottomrule
\end{tabular} \label{table4:term}
\end{table}
